ConfEx: A Framework for Automating Text-based Software Configuration Analysis in the Cloud

Modern cloud services have complex architectures, often comprising many software components, and depend on hundreds of configurations parameters to function correctly, securely, and with high performance. Due to the prevalence of open-source software, developers can easily deploy services using third-party software without mastering the configurations of that software. As a result, configuration errors (i.e., misconfigurations) are among the leading causes of service disruptions and outages. While existing cloud automation tools ease the process of service deployment and management, support for detecting misconfigurations in the cloud has not been addressed thoroughly, likely due to the lack of frameworks suitable for consistent parsing of unstandardized configuration files. This paper introduces ConfEx, a framework that enables discovery and extraction of text-based software configurations in the cloud. ConfEx uses a novel vocabulary-based technique to identify configuration files in cloud system instances with unlabeled content. To extract the information in these files, ConfEx leverages existing configuration parsers and post-processes the extracted data for analysis. We show that ConfEx achieves over 99% precision and 100% recall in identifying configuration files on 7805 popular Docker Hub images. Using two applied examples, we demonstrate that ConfEx also enables detecting misconfigurations in the cloud via existing tools that are designed for configurations represented as key-value pairs, revealing 184 errors in public Docker Hub images.

==> cover.tex <==
\vspace{0.5in}

\noindent Dear Editors,\\

We are submitting the attached paper, ``ConfEx: A Framework for Automating Text-based Software Configuration Analysis in the Cloud", to the IEEE Transactions on Cloud Computing (TCC).
This paper introduces a novel way of systematically analyzing text-file based software configurations in the cloud and, in this way, aims to improve the utility of (mis)configuration analytics for achieving a more secure, efficient, and reliable cloud environment.\\

The work presented in this paper is a significantly expanded and revised version of {\it
``ConfEx: Towards Automating Software Configuration Analytics in the Cloud''}, which was authored by Ozan Tuncer, Nilton Bila, Sastry Duri, Canturk Isci, and Ayse K. Coskun, and accepted for publication at the ``International Conference on Dependable Systems and Networks (DSN'18)'' (attached for your convenience). 
In our DSN'18 paper, we introduced ConfEx, a framework that enables discovery and analysis of text-based configurations in  the cloud.
%
%
%
\\

In this submission, we enhance our framework to systematically collect an extended set of configuration-related information from cloud instances (i.e., VMs, containers, or images), enabling deeper analysis.
Our improved framework allows focusing on configurations that are actively used in cloud instances and allows the detection of a wider set of misconfigurations.
%
In particular, this TCC paper includes the following new material:

\begin{itemize}

\item Our current paper introduces two methods to isolate active configurations and reduce false positives in misconfiguration detection algorithms.
Our first method uses system call logs collected during application initialization to determine what configuration files are in use. Our second method targets platforms where system call logs are not readily available and uses the Linux file access timestamps.

\item Our enhanced framework collects and analyzes environmental information (e.g., file metadata, environmental variables) and the order of parameters in configuration files to enable detection of a wider set of misconfigurations, including missing file permissions and invalid parameter ordering.

\item This submission expands the uses cases supported by our framework. In our DSN'18 paper, we showed that the framework supports detection of misconfigurations in images with a single configuration error using the PeerPressure~\cite{Wang:OSDI04:peerPressure} algorithm. In this submission, we show that ConfEx can be used to detect multi-parameter inconsistencies and inconsistencies between parameters and the environment. To this end, we implement and evaluate the Encore~\cite{Zhang:ASPLOS14:encore} algorithm using our ConfEx framework.

\end{itemize}

\vspace{0.1in}

In summary, our enhancements to ConfEx and our extended evaluation represent substantial novelty in terms of new research and experimental analysis compared to our DSN'18 conference paper.
All results, figures, and tables in the paper except for Figure~\ref{fig:framework:discovery} and Table~\ref{tab:real_misconfigs} are completely new.\\

We believe that this new material makes a much stronger contribution to the
literature, as our extended framework leads to a more comprehensive and robust analysis of text-based software configurations in cloud instances.\\ 

\vspace{0.4in}
Sincerely,

\vspace{0.1in}
\noindent Ozan Tuncer, Nilton Bila, Sastry Duri, Canturk Isci, and Ayse K. Coskun

\vspace{0.1in}
\noindent{Contact Author: Ozan Tuncer (otuncer@bu.edu)}


